ROBUS: Fair Cache Allocation for Multi-tenant Data-parallel Workloads

Systems for processing big data---e.g., Hadoop, Spark, and massively parallel databases---need to run workloads on behalf of multiple tenants simultaneously. The abundant disk-based storage in these systems is usually complemented by a smaller, but much faster, {\em cache}. Cache is a precious resource: Tenants who get to use cache can see two orders of magnitude performance improvement. Cache is also a limited and hence shared resource: Unlike a resource like a CPU core which can be used by only one tenant at a time, a cached data item can be accessed by multiple tenants at the same time. Cache, therefore, has to be shared by a multi-tenancy-aware policy across tenants, each having a unique set of priorities and workload characteristics. In this paper, we develop cache allocation strategies that speed up the overall workload while being {\em fair} to each tenant. We build a novel fairness model targeted at the shared resource setting that incorporates not only the more standard concepts of Pareto-efficiency and sharing incentive, but also define envy freeness via the notion of {\em core} from cooperative game theory. Our cache management platform, ROBUS, uses randomization over small time batches, and we develop a proportionally fair allocation mechanism that satisfies the core property in expectation. We show that this algorithm and related fair algorithms can be approximated to arbitrary precision in polynomial time. We evaluate these algorithms on a ROBUS prototype implemented on Spark with RDD store used as cache. Our evaluation on a synthetically generated industry-standard workload shows that our algorithms provide a speedup close to performance optimal algorithms while guaranteeing fairness across tenants.

==> concepts.tex <==
\section{Concepts}

\subsection{CPU Fair Share Schedulers: Overview}

\subsection{Shark/ Spark}

\begin{itemize}
 \item We plan to use a single Shark context with fair share task scheduler. This enables us to manage entire memory ourselves without partitioning it.
\end{itemize}

Questions:
\begin{enumerate}
 \item Should we consider Tachyon which allows memory to be shared across multiple Spark applications and have a separate context per pool? However, Tachyon is rather immature at this stage and we might run into issues setting it up. 
\end{enumerate}

\subsection{Managing Shark Cache for Efficiency}

Components

Generator:
- generates queries with a Poisson distribution. Parameter used: $\lambda$, rate of generation
- assigns a queue for every generated query. Parameter used: $\gamma$, probability distribution of queries to queue. This will help us recreate practical scenarios like more queries assigned to production queue than development queue.
- uses datasets of certain sizes that go well with available RDD memory. We have pre-defined clusters of columns(to be used as grouping columns) clustered by their size. Parameter used: $\delta$, probability distribution over the clusters of columns.
- ensures that a sequence of queries generated share grouping columns. What we desire is a guarantee like "any sequence of 'n' queries contains 'n/p' distinct grouping columns with high probability". Here 'p' is a parameter that controls sharing. Not sure how to provide this guarantee as of now. Harold's implementation generated a fixed number of queries at a time and used two parameters to control which datasets to use and where to place the queries in queues respectively. This won't help us since: (a) query generation is a continuous process here, and (b) it is desired that sharing is independent of batching.
- randomly picks a set of columns from the dataset containing the grouping column and adds aggregations over them. Parameter used: $\zeta$, average number of aggregations per query.
- fires an event queryGenerated(QueryID). This is useful for monitoring.

Queue:
- A wrapper over a queue/pool/buffer object.
- Provides an API fetchABatch() that pops a batch of queries from the buffer and returns as an ordered list. (parameter: batch size 'B')
- While returning a batch, fires an event queryFetchedByCachePlanner(QueryID) for each query. This will help us find how long, on average, queries in each queue have to wait in external queue.

CachePlanner:
- Multiple implementations are possible. e.g. A lazy CachePlanner would wait till all previously scheduled jobs to finish before looking at a new batch of queries or an aggressive CachePlanner would start processing new batch as soon as it has scheduled all queries from previous batch. More details in a separate discussion.
- Provides a method called analyzeBatch(List<Batch>). It receives a batch of queries from each queue retrieved using fetchABatch() API (returning <=B queries). 
- Translates a query to HiveQL while pushing to Spark's internal scheduler. Also fires an event queryPushedToSharkScheduler(QueryID).
- Have to treat caching query differently since it may use combined queues separately and has to be monitored as part of queries that will be helped by it.

Data Structures:

Query object:
- QueryID
- QueueID
- Grouping column
- Selectivity conditions
- Set of aggregations

Queue object:
- QueueID
- Weight
- Min share (set to 0)

Column object:
- Name
- Name of parent dataset 
- Cache size estimate 


Events tracked for monitoring:

1. Generated by CachePlanner
 a. queryGenerated
 b. queryFetchedByCachePlanner
 c. queryPushedToSharkScheduler

2. Generated by Shark/Spark
 a. stageStarted 
 b. stageFinished
Shark events are per stage and we need a mapping to our query object. It can be extracted from stage description that Shark provides.

Overview:
\begin{itemize}
 \item Do not expose Shark's internal queues, but rather have equivalent external queues to buffer incoming queries. Each pool has a weight associated, all weights add up to 100\%. Min share of each pool is set to 0. Weights of internal pools is subject to change for performance reasons, will be elaborated later.
 \item The performance optimization we want to try is materializing common sub-expression. First cut would just consider single column grouping and aggregation queries (of the form `SELECT AGG(A) from R GROUP BY B') and look for exact matches to materialize.
 \item Algorithm will look at a batch of queries in external queues and try to find out the best set of columns that fit the memory and give most benefits. (Quantifying benefits is part of algorithm's logic.)
 \item A caching query that benefits multiple queues is executed with combined shares of the queues. We change Shark's pool configuration before putting the caching query to internal queues and once it finishes, we revert the configuration back.
\end{itemize}

Questions:
\begin{enumerate}
 \item How to estimate cached data size? Should we assume existence of prediction models initially till we get main algorithm working.
 \item What is a batch? We could invoke the algorithm after a fixed period in time. But we also need to make sure that all previously scheduled queries are finished so that we do not have to worry about cache evictions. If we are looking at a fixed length batch, we would still have to wait for queries from previous batch that depend on cached datasets before firing any caching query.
 \item How does Shark handle dynamic changes to pool configuration? Can we, for example, change configuration of two of three pools without affecting any running queries in the third pool or does it need a reset of all the pools?
\end{enumerate}


\subsection{Notions of Fairness}

For each of the notions, we will first describe how it applies to internal task scheduler and how we interpret it for external cache planner. 

\subsubsection{Resource-based}

\begin{itemize}
 \item Due to delays in task scheduling due to resource unavailability, jobs may not get fair share of resources at all times. We assume here that the share is defined for the number of CPU cores i.e. resource is uni-dimensional. The unfairness in the system can be computed using Jain's index~\cite{jain} which gives a fairness score between 0 and 1 depending on the variance in fair allocation and actual allocation.
 \item In our setting, we want to guarantee the same fairness on external queues. Internally, we combine queues from time-to-time for materialization queries. Whenever we do this, we need a mapping of external queue and corresponding internal queue while monitoring. If an external queue is mapped to a combined queue internally and if the combined queue is receiving more than the external queue's stipulated resources, the allocation is deemed fully fair. We do not factor in fair share of internal queue in computation although we set them to be the same as sum of shares of combined queues.
\end{itemize}

\subsubsection{Performance-based}

\begin{itemize}
 \item For task schedulers, performance-based fairness is defined in terms of variance in slowdowns of jobs in shared cluster compared to a baseline case where every job receives all the resources. Quincy~\cite{quincy} defines this metric as a coefficient of variation of all `Application normalized performances'(ANPs). ANP of a job is defined in ~\cite{anp} as the ratio of its execution time in ideal condition to its execution time in shared cluster.
 \item The above notion compares relative slowdowns in jobs in queues. However, our cache planner is trying to enhance the performance and therefore, we would like to compare relative speed-ups across queues. The baseline for us would be the case of no caching. We then employ our cache planner algorithm on the same workload and compute inverse speed-ups of all jobs. The unfairness is a coefficient of variation of these ratios.
\end{itemize}



Questions:
\begin{enumerate}
 \item Do we need to compute unfairness index for every queue or just one single overall number is sufficient?
 \item Is uni-dimensional fairness good enough? Or should we also include memory in fair share definition?
\end{enumerate}

==> discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}

Online ROBUS or artificial wait for best effort(lower priority) jobs

Different options exist: profiling used to predict query workload which will retain certain views.

Combined cost model, trade-off one resource for another
